A Runtime Environment for Contract Automata

Contract automata have been introduced for specifying applications through behavioural contracts and for synthesising their orchestrations as finite state automata. This paper addresses the realisation of applications from contract automata specifications. We present CARE, a new runtime environment to coordinate services implementing contracts that guarantees the adherence of the implementation to its contract. We discuss how CARE can be adopted to realise contract-based applications, its formal guarantees, and we identify the responsibilities of the involved business actors. Experiments show the benefits of adopting CARE with respect to manual implementations.

==> BobInterface.tex <==

\begin{minted}[mathescape,linenos,fontsize=\scriptsize]{java}
public interface BobInterface {
    public String coffee(Integer sugar); public String tea(Integer sugar);
    public String euro(Integer money); public String dollar(Integer money); }
\end{minted}

==> macros.tex <==
%\usepackage{newtxtext,newtxmath}
\usepackage{amsmath,amssymb,amstext} %,latexsym}
\usepackage[misc]{ifsym}
%\usepackage{pifont}
%\newcommand{\cmark}{\text{\ding{51}}}
%\newcommand{\xmark}{\text{\ding{55}}}
%\usepackage{stmaryrd}
%\usepackage{wasysym}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{booktabs,colortbl}
\usepackage{wrapfig}

% For Springer
\makeatletter
\RequirePackage[bookmarks,unicode,colorlinks=true]{hyperref}%
   \def\@citecolor{blue}%
   \def\@urlcolor{blue}%
   \def\@linkcolor{blue}%
\def\UrlFont{\rmfamily}
\def\orcidID#1{\smash{\href{http://orcid.org/#1}{\protect\raisebox{-1.25pt}{\protect\includegraphics{orcid_color.eps}}}}}
\makeatother

\usepackage[capitalise]{cleveref}

\usepackage{doi,url}

\usepackage{todonotes}

%%
%		MACRO CONDIVISE
%%
%%%


\newcommand{\prset}{\texttt{Pr}}

\newcommand{\uncdis}{U_{p\mathcal A\mathcal K_n}} 

\newcommand{\Alice}{\textit{Alice\/}}
\newcommand{\Bob}{\textit{Bob\/}}
\newcommand{\Carol}{\textit{Carol\/}}

\newcommand{\deprecated}[1]{ \color{brown} {\small #1} \color{black}}

\newcommand{\toremove}[1]{ \color{gray} \sout{#1} \color{black}}

%%%%% acta vecos

\usepackage{xifthen}
\newcommand{\inv}[1][]{%
\ifthenelse{\equal{#1}{}}{I}{I(#1)}%
}
\newcommand{\con}[1][]{%
\ifthenelse{\equal{#1}{}}{\chi}{\chi(#1)}%
}

%%%%% urgent, greedy, lazy requests

\newcommand{\xor}{\oplus}
\newcommand{\acronym}{MSCA}
\newcommand{\permittedset}{A^{\Diamond}}
\newcommand{\necessaryset}{A^{\Box}}
\newcommand{\urgentset}{A^{\Box_u}}
\newcommand{\greedyset}{ A^{\Box_g}}
\newcommand{\lazyset}{A^{\Box_{\ell}}}
\newcommand{\offerset}{A^o}
\newcommand{\Boxurgent}{\Box_{\textit{unc\/}}}
\newcommand{\Boxlazy}{\Box_{\ell}}
\newcommand{\Permitted}{\Diamond}
\newcommand{\permitted}{$\Diamond$}
\newcommand{\necessary}{$\Box$}

%%%% may, must

\newcommand{\may}{\textit{may }}
\newcommand{\must}{\textit{must }}
\newcommand{\mpc}{\textit{mpc}}

%%%%%%%%%%
% CAT
\newcommand{\myconf}[1]{\langle #1 \rangle}
\newcommand{\ampl}{\texttt{AMPL}}
\newcommand{\CA}{\texttt{CA}}
\newcommand{\CATransition}{\texttt{CATransition}}
\newcommand{\CAUtil}{\texttt{CAUtil}}
\newcommand{\tool}{\textsf{FMCAT}}
\newcommand{\jamata}{\textsf{JA}}
\newcommand{\ca}{CA}
\newcommand{\code}[1]{\mbox{\texttt{#1}}}
\newcommand{\codes}[1]{\mbox{\small{\texttt{#1}}}}
%%%%%%%%%%%

\newcommand{\alert}[1]{ \color{red} #1 \color{black} }
\newcommand{\mobius}{M{\"o}bius }

%%%%%%%%%%%
% CA and so on
\newcommand{\redset}[1]{\mathit{edundant}({#1})}
\newcommand{\liable}[1]{\mathit{SLiable}({#1})}
\newcommand{\tliable}[1]{\mathit{TSLiable}({#1})}

\newcommand{\chanset}{C}
\newcommand{\ithel}[2]{{#1}_{({#2})}}
\newcommand{\ithelprime}[2]{{#1}\,'_{\!({#2})}}
%\newcommand{\blk}{\text{\textvisiblespace}}
%\newcommand{\blk}{\mbox{\small$\star$}}%\usepackage{stmayrd}
\newcommand{\blk}{\bullet}
\newcommand{\Oset}{\mathsf{O}}
\newcommand{\Rset}{\mathsf{R}}
\newcommand{\Lset}{\mathsf{L}}
\newcommand{\matchrel}{\Join}
\newcommand{\aca}[1]{\mathcal{#1}}
%\newcommand{\conf}[1]{\langle{#1}\rangle}
\newcommand{\proj}[2]{\mathtt{proj}_{#1}({#2})}
\newcommand{\ASigma}{\Rset \cup \Oset}

\newcommand{\projg}[2]{#1 \downharpoonright \ptp #2}

\newcommand{\projo}[1]{#1 \!\!\downharpoonright_\Oset}

\newcommand{\projop}[2]{#1 \!\!\downharpoonright_{\Oset, \ptp #2}}

\newcommand{\GSet}{\mathcal{G}}
\newcommand{\PSet}{\!\mathcal{P}\!}
\newcommand{\NSet}{\!\mathcal{N}\!}

\newcommand{\mmdef}{\overset{{\text{def}}}{=}}
%\newcommand{\mmdef}{=}   %uso questo l'altro spesso non lo uso
\newcommand{\define}{\triangleq}

\newcommand{\aset}[1]{\langle{#1}\rangle}
\newcommand{\ASET}[1]{\{ {#1} \}}

\newcommand{\st}{\;\big|\;} %such that set

\newcommand{\action}{\ell}

%\newcommand{\co}{\overline}

\newcommand{\TRANS}[1]{\xrightarrow{#1}}
\newcommand{\TRANSX}[1]{\stackrel{#1}{\rightsquigarrow}}
\newcommand{\TRANSS}[1]{{\xrightarrow{\raisebox{-.3ex}[0pt][0pt]{\scriptsize $#1$}}}}

\newcommand{\TRANSOB}[1]{\stackrel{#1}{\twoheadrightarrow}}

\newcommand{\NTRANSS}[1]{\not\!\xrightarrow{\raisebox{-.3ex}[0pt][0pt]{\scriptsize $#1$}}}
\newcommand{\TRANSAST}[1]{\stackrel{#1}{\R^\ast}}

\newcommand{\TAUTRANS}[1]{\stackrel{#1}{\Longrightarrow}}

\newcommand{\TRANSs}[1]{\stackrel{#1}{\R}_\ocircle}

\newcommand{\TAUTRANSs}[1]{\stackrel{#1}{\Longrightarrow}_\ocircle}

\newcommand{\TAUTRANSS}[1]{\smash{\overset{\raisebox{-.4ex}{\scriptsize $#1$}}{\Longrightarrow}}}

% Reduction
\newcommand{\osred}{\rightarrow}                % one-step reduction relation
\newcommand{\R}{\osred}
\newcommand{\msred}{\osred^\ast}     % multi-step reduction
\newcommand{\RR}{\msred}

\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\thmref}[1]{Theorem~\ref{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\newcommand{\dummy}{\psframe[linecolor=white,fillstyle=solid,fillcolor=lightgray](0.05,-0.05)(0.35,0.25) \hspace{0.4cm}}

\renewcommand{\epsilon}{\varepsilon}
\newcommand{\setenum}[1]{\{#1\}}
\newcommand{\setcomp}[2]{\{\, #1 \mid #2 \,\}}
\newcommand{\powset}[1]{2^{#1}}
\newcommand{\glb}{\sqcap}
\newcommand{\lub}{\sqcup}
\newcommand{\lra}{\longrightarrow}
\newcommand{\absedge}[1]{\xrightarrow{#1}}

\newcommand{\eqdef}{\triangleq}

\newcommand{\Nat}{\mathit{Nat}}
\newcommand{\Int}{\mathit{Int}}
\newcommand{\Bool}{\mathit{Bool}}
\newcommand{\true}{\mathit{tt}}
\newcommand{\false}{\mathit{ff}}

\newcommand{\Ev}{\ensuremath{\textsf{Ev}}}
\newcommand{\Pol}{\ensuremath{\textsf{Pol}}}
\newcommand{\Frm}{\ensuremath{\textsf{Frm}}}
\newcommand{\Cls}{\ensuremath{\textsf{Cls}}}
\newcommand{\Srv}{\ensuremath{\textsf{Srv}}}
\newcommand{\Comm}{\ensuremath{\textsf{Comm}}}
\newcommand{\Req}{\ensuremath{\textsf{Req}}}
\newcommand{\Loc}{\ensuremath{\textsf{Loc}}}
\newcommand{\Act}{\ensuremath{\textsf{Act}}}

\newcommand{\plan}[1]{\setenum{#1}}
\newcommand{\sframe}[2]{#1[#2]}
\newcommand{\lframe}[2]{#1\langle #2 \rangle}
\newcommand{\llframe}[2]{#1\langle\!\langle #2 \rangle\!\rangle}
\newcommand{\ifthen}[3]{\texttt{if}\hspace{2pt}#1\hspace{2pt}\texttt{then}\hspace{2pt}#2 \hspace{2pt} \texttt{else} \hspace{2pt} #3}
\newcommand{\unavail}[0]{\textsf{N/A}}
\newcommand{\letin}[2]{\textup{\texttt{let}} \hspace{3pt} #1 \,\textup{\texttt{in}} \hspace{3pt} #2}

\newcommand{\branch}{\texttt{branch}}

\newcommand{\fail}{\texttt{fail}}
\newcommand{\wait}[1][]{\texttt{wait} \, #1}
\newcommand{\try}[2]{\texttt{try}\hspace{2pt}#1\hspace{2pt}\texttt{with}\hspace{2pt}#2}
\newcommand{\rrangle}[0]{\mbox{\ensuremath{\rangle\hspace{-2pt}\rangle}}}

\newcommand{\fv}[1]{\mathit{fv}(#1)}
\newcommand{\BPA}[1]{\mathit{BPA}(#1)}
% \newcommand{\unit}[0]{\mathit{unit}}
%\newcommand{\unit}[0]{1}

\newcommand{\wnorm}[2]{#1 \!\downarrow_{#2}}
\newcommand{\snorm}[2]{#1 \!\Downarrow_{#2}}
\newcommand{\guard}[2]{\mathit{guard}(#2)}
%\newcommand{\hole}[0]{\bullet}
\newcommand{\valid}[1]{\models #1}
% \newcommand{\linear}[1]{\mathit{lin}(#1)}
\newcommand{\linear}[1]{\Lambda(#1)}

\newcommand{\abs}[1]{#1^\sharp}
\newcommand{\sem}[3][]{\mbox{\ensuremath{\llbracket#2\rrbracket_{#3}^{#1}}}}
\newcommand{\Sem}[2][]{\mbox{\ensuremath{\langle\!\langle#2\rangle\!\rangle^{#1}}}}
\newcommand{\bind}[2]{#2 / #1}
\newcommand{\emptystack}{[\hspace{1pt}]}
\newcommand{\seq}[1]{(#1)}
\newcommand{\pair}[2]{(#1,#2)}
\newcommand{\lift}[1]{{}_{\llcorner}\hspace{-2pt} #1 \hspace{-1pt}{}_{\lrcorner}}
\newcommand{\irule}[2]{\frac{\textstyle\rule[-1.3ex]{0cm}{3ex}#1}%
{\textstyle\rule[-.5ex]{0cm}{3ex}#2}}

\newcommand{\hbra}{
\hbox to 1 \textwidth{\vrule width0.3mm height 1.8mm depth-0.3mm
                    \leaders\hrule height1.8mm depth-1.5mm\hfill
                    \vrule width0.3mm height 1.8mm depth-0.3mm}}
\newcommand{\hket}{
\hbox to 1 \textwidth{\vrule width0.3mm height1.5mm
                    \leaders\hrule height0.3mm\hfill
                    \vrule width0.3mm height1.5mm}}

\newcommand{\lambdabox}{\ensuremath{\lambda^{[\,]}\;}}
\newcommand{\lambdareq}{\ensuremath{\lambda^{\mathit{req}\;}}}
\newcommand{\frbox}{{\ensuremath{[\,]}}}
\newcommand{\frdiamond}{{\ensuremath{\langle\,\rangle}\!}}

\newcommand{\srv}[2]{#1 \langle #2 \rangle}
\newcommand{\res}[2]{#1 / #2}

\newcommand{\open}[2][]{\texttt{open}_{#1} #2}
\newcommand{\close}[2][]{\texttt{close}_{#1} #2}
\newcommand{\listen}[2][]{\texttt{listen}_{#1} #2}

\newcommand{\qst}{\;\colon\;} %such that logic

\newcommand{\A}{\bold{A}}

\newcommand{\Abot}{\bold{A^\bot}}

\newcommand{\La}{\bold{L}}

\newcommand{\illmix}{$ILL^{mix}$}

\newcommand{\aout}{\overline{a}}
\newcommand{\areq}{a}
\newcommand{\cout}{\overline{c}}
\newcommand{\creq}{c}
\newcommand{\dout}{\overline{d}}
\newcommand{\dreq}{d}
\newcommand{\okout}{\overline{ok}}
\newcommand{\okreq}{ok}

\makeatletter
\def\thickhline{%
  \noalign{\ifnum0=`}\fi\hrule \@height \thickarrayrulewidth \futurelet
   \reserved@a\@xthickhline}
\def\@xthickhline{\ifx\reserved@a\thickhline
               \vskip\doublerulesep
               \vskip-\thickarrayrulewidth
             \fi
      \ifnum0=`{\fi}}
\makeatother
\newlength{\thickarrayrulewidth}
\setlength{\thickarrayrulewidth}{2\arrayrulewidth}


\newcommand{\quo}[1]{\lq\lq {#1}\rq\rq}
\usepackage[most]{tcolorbox}
\newtcolorbox{markbox}{
  enhanced,
  breakable,
  size=minimal,
  parbox=false,
  after={\par},
  before upper={\indent},
  colback=white,
  overlay = {
	 \draw[line width=2pt]
	 (frame.north east) -| ([xshift=3mm]frame.east) |-(frame.south east);
  },
  overlay first={\draw[line width=2pt] (frame.north east) -| ([xshift=3mm]frame.south east);},
  overlay middle={\draw[line width=2pt] ([xshift=3mm]frame.north east) -- ([xshift=3mm]frame.south east);},
  overlay last={\draw[line width=2pt] ([xshift=3mm]frame.north east) |- (frame.south east);},
}


\newcommand{\Maucomm}[2][check]{
  \todo[fancyline,color=orange!10]{\tiny Mau: \color{orange}#1}
%  \begin{markbox}
	 {\color{OliveGreen}{#2}}
%  \end{markbox}
}

\usepackage{wrapfig}

\usepackage{lipsum}  

\setlength{\textfloatsep}{10pt plus 1.0pt minus 2.0pt}
